Minimax Optimal Online Imitation Learning via Replay Estimation

Online imitation learning is the problem of how best to mimic expert demonstrations, given access to the environment or an accurate simulator. Prior work has shown that in the infinite sample regime, exact moment matching achieves value equivalence to the expert policy. However, in the finite sample regime, even if one has no optimization error, empirical variance can lead to a performance gap that scales with $H^2 / N$ for behavioral cloning and $H / \sqrt{N}$ for online moment matching, where $H$ is the horizon and $N$ is the size of the expert dataset. We introduce the technique of replay estimation to reduce this empirical variance: by repeatedly executing cached expert actions in a stochastic simulator, we compute a smoother expert visitation distribution estimate to match. In the presence of general function approximation, we prove a meta theorem reducing the performance gap of our approach to the parameter estimation error for offline classification (i.e. learning the expert policy). In the tabular setting or with linear function approximation, our meta theorem shows that the performance gap incurred by our approach achieves the optimal $\widetilde{O} \left( \min({H^{3/2}} / {N}, {H} / {\sqrt{N}} \right)$ dependency, under significantly weaker assumptions compared to prior work. We implement multiple instantiations of our approach on several continuous control tasks and find that we are able to significantly improve policy performance across a variety of dataset sizes.

==> checklist.tex <==
% \section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%

%%% END INSTRUCTIONS %%%



% \begin{enumerate}


% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}


% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerYes{}
%         \item Did you include complete proofs of all theoretical results?
%     \answerYes{}
% \end{enumerate}


% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{}
%         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerYes{}
%         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{}
% \end{enumerate}


% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerYes{}
%   \item Did you mention the license of the assets?
%     \answerYes{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%   \answerYes{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerYes{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerNA{}
% \end{enumerate}


% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}


% \end{enumerate}

==> defs-icml.tex <==
\usepackage{bbm}
\usepackage{graphicx}
\usepackage{amsmath,amssymb,amsthm,amsfonts}

\usepackage{paralist}
\usepackage{bm}
\usepackage{xspace}
\usepackage{url}
\usepackage{prettyref}
\usepackage{boxedminipage}
\usepackage{wrapfig}
\usepackage{ifthen}
\usepackage{color}
\usepackage{xspace}

\newcommand{\ii}{{\sc Indicator-Instance}\xspace}
\newcommand{\midd}{{\sf mid}}


\usepackage{amsmath,amsthm,amsfonts,amssymb}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{graphicx}


% \usepackage{fullpage}
\usepackage{hyperref}
\usepackage{nicefrac}

\newtheorem{inftheorem}{Informal Theorem}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\usepackage{subcaption}

\newtheorem{problem}{Problem}
\usepackage[utf8]{inputenc}
\newcommand{\nived}[1]{{\color{red}{\small{\bf [Nived: #1]}}}}
\newcommand{\ceil}[1]{\lceil#1\rceil}
\newcommand{\rank}{\mathsf{rank}}
\newcommand{\tr}{\mathsf{Tr}}
\newcommand{\tv}{\mathsf{TV}}
\newcommand{\opt}{\mathsf{OPT}}
\newcommand{\rr}{\textsc{R}\space}
\newcommand{\alg}{\textsf{Alg}\space}
\newcommand{\sd}{\textsf{sd}_\lambda}
\newcommand{\lblq}{\mathfrak{lq} (X_1)}
\newcommand{\diag}{\textsf{diag}}
\newcommand{\sign}{\textsf{sgn}}
\newcommand{\BC}{\texttt{BC} }
\newcommand{\MM}{\texttt{MM} }
\newcommand{\Nexp}{N_{\mathrm{exp}}}
\newcommand{\Nrep}{N_{\mathrm{replay}}}
\newcommand{\Drep}{D_{\mathrm{replay}}}
\newcommand{\Nsim}{N_{\mathrm{sim}}}
\newcommand{\piBC}{\pi^{\texttt{BC}}}
\newcommand{\piRE}{\pi^{\texttt{RE}}}
\newcommand{\piEMM}{\pi^{\texttt{MM}}}
\newcommand{\mmd}{\texttt{Mimic-MD} }
\newcommand{\RE}{\texttt{RE} }
\newcommand{\dem}{\pi^E}
\newcommand{\Rlint}{\mathcal{R}_{\mathrm{lin,t}}}
\newcommand{\Rlipt}{\mathcal{R}_{\mathrm{lip,t}}}
\newcommand{\Rlin}{\mathcal{R}_{\mathrm{lin}}}
\newcommand{\Rlip}{\mathcal{R}_{\mathrm{lip}}}
\newcommand{\Rmax}{R_{\mathrm{max}}}
\newcommand{\Rall}{\mathcal{R}_{\mathrm{all}}}
\newcommand{\Rdet}{\mathcal{R}_{\mathrm{det}}}
\newcommand{\Fmax}{F_{\mathrm{max}}}
\newcommand{\piref}{\pi^{\mathrm{ref}}}
\newcommand{\green}{\text{\color{green!75!black} green}\;}
\newcommand{\red}{\text{\color{red} red}\;}
\newcommand{\blue}{\text{\color{blue} blue}\;}
\newcommand{\thetaBC}{\widehat{\theta}^{\textsf{BC}}}
\newcommand{\ent}{\mathcal{E}_{\Theta_t,\Nexp,\delta}}
\newcommand{\entH}{\mathcal{E}_{\Theta_t,\Nexp,\delta/H}}

\usepackage{xcolor}

\usepackage{thmtools}
\usepackage{thm-restate}

==> morally-det.tex <==
What happens when the expert is approximately optimal?

First we begin with a setting where the expert is a "noisy" optimal policy. 

\begin{definition} \label{def:noisyopt}
Suppose for every $(s,a,t)$ tuple,
\begin{align}
    \tv \left( \dem_t (s,a), \pi^*_t (s,a) \right) \le \gamma
\end{align}
where $\pi^*$ is an optimal policy on the IL instance.
\end{definition}

\begin{theorem}
For any $\gamma \ge 0$ there exists an IL instance with a $\gamma$-noisy optimal expert such that if $N \le 2^H$, with constant probability, for any learner in the no-interaction or known-transition settings,
\begin{align}
    J(\dem) - J (\widehat{\pi}) \gtrsim \frac{H}{\sqrt{N}}.
\end{align}
\end{theorem}

Consider an IL instance with the following structure. The MDP is deterministic with the transition induced by different actions labelled by different colors. The reward function of the MDP is sampled from a distribution, which is given below,
\begin{align}
    &r_t (\red | s=5) \sim \mathrm{Unif}  (\{ 0,1 \}) \\
    &r_t (\red | s=6) = 1 - r_t (\red | s=5) \\
    &r_t (\red | s=3) \sim \mathrm{Unif}  (\{ 0,\frac{1}{3} \})  \\
    &r_t (\red | s=1) = \frac{1}{3} - r_t (\red | s=3) \\
\end{align}
In other words, only one of state $1$ or $3$ offers rewards until time $H/2$. And subsequently from time $H/2+1$ onwards, states $5$ and $6$ may also be visited, again, only one of which offers rewards.

The optimal policy on this MDP is simple to compute - $\pi^*$ simply picks the \green action at state $2$ until time $H/2$ and then picks either the \red or \blue action depending on whether $r_t (\red | s=5) = 1$ or $r_t (\red | s=6) = 1$ (recall that only one of these rewards is $1$, and the other is $0$).

Now we specify the expert's policy. Recall that the expert is a noisy version of the optimal policy. At states all the states besides state $2$, there is only a single action to choose. All policies are equivalent on these states. However, at state $2$, the expert is stochastic and deviates from the optimal policy. At each time $2 \le t \le H/2-1$, the expert picks the \red action with probability $\gamma$ and the green action with probability $1-\gamma$. For $2 \le t \le H/2 - 1$,
\begin{align}
    \pi^*_t (\green | s=2) = 1-\gamma.
\end{align}
At time $H/2$, the expert picks the same action as the optimal policy, collecting a reward of $H/2$ then onward. On the other hand, at time $1$, the expert picks whichever action leads to the state with reward $1$. Namely, the expert is perfectly correlated with the random reward function in such a way that,
\begin{align}
    \pi^*_{H/2} (\red|s) =
    \begin{cases}
        \frac{1}{2} \qquad &r_t (\red | s=3) \ne 0 \\
        0 &\text{otherwise.}
    \end{cases}
\end{align}
Finally, at the state $s=2$ at time $t=1$,
\begin{align}
    \pi^*_1 (\cdot|s=2) = 
\end{align}

Recall the assumption that, $H \ge 2\log_{\frac{1}{1-\gamma}} (N)$. From here, we have that,
\begin{align}
    (1 - \gamma)^{H/2} \le \frac{\delta}{N}.
\end{align}
Note that the LHS is the probability that the expert reaches state $2$ at time $H/2$ in a single rollout. The interpretation is that under the optimal policy $\pi^*$, the state $2$ is visited with probability $1$ at time $H/2$. However, under the expert policy, the probability of visiting is very small, and at most $\delta/N$. Therefore, with probability $(1 - 1/N)^N \ge \frac{1}{4}$ over the dataset, the state $2$ is never visited at time $H/2$ in the dataset. Under this event, even with the knowledge of the transition, the learner cannot know what action to play at state $2$ at time $H/2$. Thus the learner may incorrectly choose to visit the state among $5$ and $6$ which offers no reward and potentially lose out on a significant amount of reward.

Define the event $\mathcal{E}_1$ as the event that state $2$ is never visited at time $H/2$ in any of the trajectories of the expert dataset. Then,
\begin{align}
    \mathrm{Pr} (\mathcal{E}_1) \ge 1/4
\end{align}
Recall that the expert policy is sampled from a distribution. This is defined as,
\begin{align}
    s
\end{align}


\begin{figure}[h!]
\centering
\begin{tikzpicture}[shorten >=1pt,node distance=1.25cm,on grid,auto,good/.style={circle, draw=black!60, fill=green!30!white, thick, minimum size=9mm, inner sep=0pt},bad/.style={circle, draw=black!60, fill=red!30, thick, minimum size=9mm, inner sep=0pt}]
\tikzset{every edge/.style={very thick, draw=red!90!black}}    \tikzset{every loop/.style={min distance=9mm,in=86,out=125, looseness=8, very thick, draw=red!90!black}}
    
\node[good]     (s2)    {$2$};
\node[good]     (s3)    [above right = 1cm and 3cm of s2]  {$3$};
\node[good]     (s2')    [above = 2.5cm of s2]  {$2$};
\node[good]     (s4')    [above right = 0.66cm and 2cm of s2']  {$4$};
\node           (dots)    [above = 3cm of s2']  {$\vdots$};
\node           (blank)    [above = 1.5cm of s2']  {};
\node[good]     (s2'')    [above = 2.5cm of dots]  {$2$};
\node           (blank')    [below = 1.5cm of s2'']  {};
% \node[good]     (s4'')    [above = 2.5cm of dots]  {$2$};
\node[good]     (s4'')    [above right = 0.66cm and 2cm of s2'']  {$4$};
\node[good]     (s2''')    [above = 2.5cm of s2'']  {$2$};
\node           (empty)    [right = 5cm of s2''']  {};
\node           (emptylabel)    [right = 0.5cm of empty]  {$t = \frac{H}{2}$};
\node           (empty')    [right = 5cm of s2'']  {};
\node           (emptylabel')    [right = 0.75cm of empty']  {$t = \frac{H}{2}-1$};
\node[good]     (s3''')    [above right = 0.66cm and 2cm of s2''']  {$6$};
\node[good]     (s1''')    [above left = 0.66cm and 2cm of s2''']  {$5$};
\node[good]     (s1)    [above left = 1cm and 3cm of s2]  {$1$};

\path[->,>=stealth]
(s2) edge [] node {} (s3)
(s2) edge [draw=blue!100!black] node {} (s1)
(s1) edge [distance=15mm,in=80,out=130, very thick] node {} (s1)
(s3) edge [distance=15mm,in=100,out=50, very thick] node {} (s3)
(s4') edge [distance=15mm,in=100,out=50, very thick] node {} (s4')
(s4'') edge [distance=15mm,in=100,out=50, very thick] node {} (s4'')
(s3''') edge [distance=15mm,in=100,out=50, very thick] node {} (s3''')
(s1''') edge [distance=15mm,in=80,out=130, very thick] node {} (s1''')
(s2') edge [] node {} (s4')
(s2') edge [] node {} (s4')
(s2'') edge [draw=green!75!black] node {} (s2''')
(s2''') edge [] node {} (s3''')
(s2'') edge [] node {} (s4'')
(s2''') edge [draw=blue!100!black] node {} (s1''')
(s2') edge[-] [draw=green!75!black] node {} (blank)
(s2''') edge[dotted,-] [draw=white!50!black] node {} (empty)
(s2'') edge[dotted,-] [draw=white!50!black] node {} (empty')
(s2'') edge[-] [draw=green!75!black] node {} (blank')
(s2) edge [draw=green!75!black] node {} (s2');
\end{tikzpicture}
\caption{}

\label{fig:mm-lowerbound}
\end{figure}

At a state which is observed $k$ times, suppose the learner always picks the action most played by the expert. Let this learner be $\widehat{\pi}$. Define the policy $\pi^{(i)}$ which plays actions according to $\pi^E$ until time $i$ and then picks actions according to $\widehat{\pi}$. Then,

\begin{align}
    J (\pi^E) - J(\widehat{\pi}) &\le \sum_{i=1}^H J (\pi^{(i)}) - J( \pi^{(i+1)}).
\end{align}
For each $i$, we bound $J (\pi^{(i)}) - J( \pi^{(i+1)})$. Indeed,
\begin{align}
    J (\pi^{(i)}) - J( \pi^{(i+1)}) = \sum_{s \in \mathcal{S}} \sum_{a \in \mathcal{A}} d^{\pi^E}_{i+1} (s) \left(  \pi^E_{i+1} (a|s) Q_{i+1}^{\pi^E} (s,a) - \widehat{\pi}_{i+1} (a|s) Q_{i+1}^{\widehat{\pi}} (s,a) \right)
\end{align}
Note that $\widehat{\pi}_{i+1} (a|s)$ picks the action most played by an expert at a state. Therefore, $\widehat{\pi}_{i+1} (a|s) = $

\section{Bounded density ratio assumption}

Here, we assume that the expert is a $\gamma$-noisy realization of the optimal policy, as defined in \cref{def:noisyopt}. In addition, we assume that, there is a bound on the average coverage of the expert policy compared to the optimal policy.

\begin{assumption}[Bounded density ratio assumption] \label{ass:1}
The optimal policy does not visit states too frequently compared to the expert policy in the following sense,
\begin{align}
    \frac{1}{H} \sum_{t=1}^H \mathbb{E}_{s \sim d_t^{\pi^*}} \left[ \frac{1}{d_t^{\dem} (s)} \right] \le C^\star |\mathcal{S}|.
\end{align}
\end{assumption}

\begin{proof}
\begin{align}
    J(\pi^*) - J(\widehat{\pi}) &= \mathbb{E}_{\pi^*} \left[ \sum_{t=1}^H r_t (s_t,a_t) \right] - \mathbb{E}_{\widehat{\pi}} \left[ \sum_{t=1}^H r_t (s_t,a_t) \right] \\
    &= \mathbb{E}_{\pi^*} \left[ \mathbb{I} (\mathcal{E}) \sum_{t=1}^H r_t (s_t,a_t) \right] - \mathbb{E}_{\widehat{\pi}} \left[ \mathbb{I} (\mathcal{E}) \sum_{t=1}^H r_t (s_t,a_t) \right] \label{eq:123000342}
\end{align}
Here, $\mathcal{E}^c$ is the event that at all states visited in the trajectory are visited at least $N_0 \triangleq \frac{1}{1-\gamma} \log(|\mathcal{S}| H/\delta)$ times. If a state is visited at least $N_0$ in the expert dataset, then with probability $\ge 1 - \frac{\delta}{|\mathcal{S}|H}$ the action played by the optimal policy at the state $s$ at time $t$, $\pi^*_t(s)$, is observed in the dataset, and is also played by $\widehat{\pi}$. Under $\mathcal{E}^c$, at all states visited in the trajectory $\{ (s_1,a_1),\cdots,(s_H,a_H) \}$, $\widehat{\pi}_t (\cdot|s_t) = \pi^*_t (\cdot|s_t)$, which results in \cref{eq:123000342}. Further upper bounding,
\begin{align}
    J(\pi^*) - J(\widehat{\pi}) &\le  H \mathbb{E}_{\pi^*} \left[ \mathbb{I} (\mathcal{E}) \right] \\
    &\le H \sum_{t = 1}^H \mathbb{E}_{\pi^*} \left[ \mathbb{I} (\mathcal{E}_t) \right] \label{eq:iop}
\end{align}
where $\mathcal{E}_t^c$ is defined as the event that the state visited at time $t$ in the trajectory is visited fewer than $N_0$ times. And therefore, $\mathcal{E} = \bigcup_{t=1}^H \mathcal{E}_t$. Next,
\begin{align}
    \mathbb{E} \left[ \mathbb{E}_{\pi^*} [\mathbb{I} (\mathcal{E}_t)] \right] &= \sum_{s \in \mathcal{S}} \left( \sum_{z=0}^{N_0-1} \binom{N}{z} \left( d^{\dem}_t (s) \right)^z \left( 1 - d^{\dem}_t (s) \right)^{N-z} \right) d_t^{\pi^*} (s) \\
    &= \sum_{s \in \mathcal{S}} \frac{d_t^{\pi^*} (s)}{d_t^{\dem} (s)} \left( \sum_{z=0}^{N_0-1} \frac{\binom{N}{z}}{\binom{N}{z+1}} \binom{N}{z+1} \left( d^{\dem}_t (s) \right)^{z+1} \left( 1 - d^{\dem}_t (s) \right)^{N-z} \right) \\
    &\overset{(i)}{\le} \sum_{s \in \mathcal{S}} \frac{d_t^{\pi^*} (s)}{d_t^{\dem} (s)} \sum_{z=0}^{N_0-1} \frac{\binom{N}{z}}{\binom{N}{z+1}} \\
    &\overset{(ii)}{=} \sum_{s \in \mathcal{S}} \frac{d_t^{\pi^*} (s)}{d_t^{\dem} (s)} \sum_{z=0}^{N_0-1} \frac{z+1}{N-z} \\
    &\le \frac{N_0^2}{N-N_0} \mathbb{E}_{s \sim d_t^{\pi^*}} \left[ \frac{1}{d_t^{\dem} (s)} \right] \label{eq:ppo}\\
\end{align}
where in $(i)$, we use the fact that $\binom{N}{z+1} x^{z+1} (1-x)^{N-z} \le 1$ for $x \in [0,1]$ (since it is a term in the binomial expansion of $(1 -x + x)^{N+1}$. In $(ii)$, we use the fact that $\frac{\binom{N}{z}}{\binom{N}{z+1}} = \frac{(z+1)! (N-z-1)!}{z! (N-z)!} = \frac{z+1}{N-z}$.
Plugging \cref{eq:ppo} into \cref{eq:iop}, we get,
\begin{align}
    \mathbb{E} \left[ J(\pi^*) - J (\widehat{\pi}) \right] &\le \frac{H N_0^2}{N - N_0} \sum_{t=1}^H \mathbb{E}_{s \sim d_t^{\pi^*}} \left[ \frac{1}{d_t^{\dem}(s)} \right] \\
    &\le C^\star \frac{H^2 N_0^2 |\mathcal{S}|}{N-N_0},
\end{align}
where the last equation follows by invoking \cref{ass:1}


\end{proof}
